Design and Implementation of a Scalable Financial Exchange in the Public Cloud

Financial exchanges are migrating to the cloud, but the best-effort nature of the public cloud is at odds with the stringent latency requirements of exchanges. We present Jasper, a system for meeting the networking requirements of financial exchanges on the public cloud. Jasper uses an overlay tree to scalably multicast market data from an exchange to ~1000 participants with low latency (250 microseconds) and a 1-microsecond difference in data reception time between any two participants. Jasper reuses the same tree for scalable inbound communication (participants to exchange), augmenting it with order pacing and a new priority queue, Limit Order Queue (LOQ), to efficiently handle bursts of market orders. Jasper achieves better scalability and 50% lower latency than the AWS multicast service. During bursty market activity, LOQ nearly doubles the order processing rate.

==> design_discussion.tex <==
\subsection{Design space discussion (just to discuss among ourselves)}

In inbound communication, there are 3 metrics we care about: (i) latency of orders, (ii) order matching rate of ME, (iii) retransmissions. 

\Para{Using Trees}
Using the trees in the reverse direction needs to be revisited. (Update: I revisited and found trees are still helpful).

Earlier we were using UDP for order submission and reducing packet drops was important. Using the tree helped reduce incast at the exchange which reduced the packet drops. 

Now we are moving to using TCP as reliable delivery is needed for order submission. Any packet drops due to incast congestion will be retransmitted. So avoiding packet drops is a second order concern where keeping low orders' latency is more important. Using proxy tree adds more hops to the path of messages, increasing the latency. So considering this and the above technique to reduce incast (assigning $B/N$ cap to each gateway), using a tree is not necessarily helpful. 

However... while using a tree LOQ can work on bigger queues and prioritize orders of one MP over the orders of another. In such a setting LOQ has more benefits compared to a per gateway LOQ. In a per gateway LOQ setting, one LOQ only has the queue formed by orders of one MP. Such a queue is shorter than a proxy queue. However, orders of one MP can still belong to diverse price levels depending on the trading strategy. In some trading strategies (e.g.,  iceberg orders, order splitting), a trader generates orders to hold several positions (i.e., price levels) in the ME's queue. Because of the diversity of prices in the orders of a single trader for a single asset, LOQ can still be helpful as it can prioritize orders closer to the mid-price over other orders. However, in a per gateway LOQ, the benefits of LOQ are going to be lesser than the benefits of LOQ+tree. 

So a question arises, does using a tree leads to enough benefits that overcome the overhead of extra hops in the path of messages? 

A tree will also decrease retransmissions which is helpful in avoiding resource wastage. 
% JINUN says: Earlier I am thinking proxy tree can help in extremely large scale. But now it seems that is not true either. Because the whole inbound direction is only doing prioritization, no aggregation/filtering, that is to say, even we add the proxy tree, the matching engine still needs to undertake the same amount of traffic finally. Of course, if proxies can do aggregation and reduce the amount of data on the fly, then that becomes another story. But here we do not have reduction of data load in the inbound direction.

\Para{Incast mitigation}
If we just use TCP, during bursts incast may occur which leads to retransmissions, which in turn leads to high latency and wastage of bandwidth. 

Avoidong incast is a desired goal.

One technique is to assign B/N egress cap to each MP. It avoids retransmission during bursts of orders. But it has a disadvantage: if one MP is using less than B/N, the other MP should be allowed to use more than B/N but this technique does not allow that

Another technique is to use ECN like technique: for example, if exchange sees that its ingress is being utilized to almost full, it sends a signal to every MP to not exceed their fair share of bandwidth (which is exchange's ingress cap divided by total number of traders). 

Look at preotego and breakwater. 

==> evaluations/throuput_evals.tex <==
% \subsection{\sysname{} Throughput}
% \label{evals_thpt}

% With our current implementation, we can exhaust $\approx$80\% of the egress bandwidth\footnote{As we try to use more egress bandwidth to reach 90-100\% utilization, VM hangs and we are currently debugging the issue} of a c2d-highcpu-8 VM on GCP. The specified VM has an egress bandwidth of 16Gbps. With 466B packets, we achieve a multicast message rate of 350K MPS. The median OML stays the same as we increase the message rate from 5K to 350K, but $99p$ increases $13\%$. In the experiment, we have 100 receivers and 10 intermediate proxies, with no VM hedging. The sender and each proxy replicate each message $F=10$ times. With 350K messages per second, the sender generates 3.5M packets per second, utilizing 81.5\% of the available egress. The VM hedging reduces the multicast rate according to the factor $H$ as each proxy replicates each multicast message $(H+1)*F$ times. 

% We use DPDK for an optimized implementation and employ zero-copy techniques to minimize the overhead of message replication. More details of our implementation are added in Appendix~\ref{app:thpt}. 

==> evaluations/trustmodels.tex <==
% \begin{table}[t]
% \centering
% \scriptsize
% \begin{tabular}{lcccc}
% \toprule
%  & \textbf{Ideal} & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} \\
%  \midrule
% \textbf{Latency (\SI{}{\micro\second})} & $0$ & $<1$ & $\approx50$ & $\approx50$ \\
% \rowcolor{lightgray}
% \textbf{Jitter (\SI{}{\micro\second})} & $0$ & $<1$ & $10+$ & $<10$ \\
% \textbf{Through-} & No & No & No & $\approx 70\%$ \\
% \textbf{put}      & Change & Change & Change & Reduced \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of \sysname{} Trust Models}
% \vspace{-0.6cm}
% \label{tab:model_comparison}
% \end{table}

% % % \vspace{-0.3cm}
% % \subsection{Performance and Security Tradeoffs}
% % \label{evals_trust_models}
% % % \vspace{-0.24cm}

% % \sysname{} trust models are evaluated based on latency, jitter and, throughput overheads. 
% % We send 8K messages per second from the hold-and-release programs to the MP's programs for 30 minutes. Jitter is calculated by measuring the difference between $90p$ and $50p$. A large jitter shows that even if simultaneous delivery/fairness is achieved at the level of hold-and-release programs, the messages experience jitter before reaching MPs which may ultimately affect the fair delivery. 

% % In model 2 and 3, the exchange and the MPs have a strict security boundary where (i) the exchange does not rely on MPs for the correctness of its operations and, (ii) the MPs do not have to reveal their trading algorithms to the exchange. In model 1, MPs are required to handover their proprietary trading algorithms to the exchnage so that it may run them and correctly follow its protocols i.e., hold-and-release. In model 2, one could assume that the the last layer of proxies serve as the gateways so no extra latency is added. However, the hold-and-release and trading programs would still be \SI{\approx50}{\micro\second} away and susceptible to latency fluctuations. 

% % Table~\ref{tab:model_comparison} summarizes the results of evaluating all 3 models. Model 1 outperforms others in performance. Model 3 is better than model 2 in jitter while model 2 is better in throughput. Model 1 already achieves fairness at the level of trading programs while model 3 can be made to do so by artificially inflating the hold-and-release deadlines by $\approx\SI{10}{\micro\second}$ to counter the jitter. For fairness with model 2, a large inflation would be required (due to latency spikes) and can be accurately found by an offline trial and error method.

==> fault_tolerance.tex <==
\section{Fault Tolerance}
\label{sec:fault_tolerance}
% \vspace{-0.24cm}

\begin{table}[!t]
\centering
\scriptsize
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{\textbf{Domain}} & \multicolumn{2}{c}{\textbf{Fault Type}} \\ \cline{2-3}
                                & \textbf{Transient} & \textbf{Long Term} \\
\midrule
\rowcolor{lightgray}
VM                              & \makecell{\{Proxy, Receiver\}\\Hedging}   & \makecell{\{Proxy, Receiver\}\\Hedging + FD} \\ \hline
Link                            & \makecell{Proxy Hedging +\\ RRPS}      & -                                \\
\bottomrule
\end{tabular}
% \vspace{-0.3cm}
\caption{\sysname{} Fault Tolerance}
\label{tab:fault_tolerance}
% \vspace{-0.3cm}
\end{table}

Table \ref{tab:fault_tolerance} summarizes how different types of faults are guarded against in \sysname{}. We do not expect long-term VM-to-VM link failures in the cloud. Similarly long term failures of on-demand VMs are not expected~\cite{gcp_sla}. However, failures of spot VMs need to be handled if we use low-cost spot VMs to decrease the dollar cost of proxies~\cite{cant_be_late_spot_vms}. However, if all proxies are spot VMs, then the entire operation of an exchange may cease as spot VMs exhibit all-or-nothing availability~\cite{cant_be_late_spot_vms}: if one spot VM becomes unavailable then it is expected that several other spot VMs will become unavailable. We may need to boot and utilize on-demand VMs until spot VMs becomes available again. Time to boot VMs vary depending on the virtualization stack and it is common to have boot times between 1s and 60s. However, starting a stopped VM is quicker than booting a new VM~\cite{quickstartvms}. Empirically, we find that starting 100 stopped c2d-highcpu-8 VMs on GCP takes $\approx\SI{20}{\second}$. So an exchange may need to stop its operation for several seconds upon any spot VMs failure. 

An alternative model designates every even-numbered proxy at each tree level as a spot VM, with the others as on-demand VMs. This setup offers cost benefits and enhances performance during failures. Proxy hedging ensures that each proxy communicates with the children of another sibling (if $H=1$). If all spot VMs become unavailable, the messages still reach their destinations because neighboring odd-numbered proxies will be active and handling communication through proxy hedging. Although this may introduce latency fluctuations, it is preferable to an approach that completely disconnects the exchange and MPs upon failures. Additionally, this model supports an efficient failure detection (FD) mechanism, as each on-demand VM can regularly check its sibling spot VM, with checks occurring frequently e.g., every $\leq\SI{0.5}{\milli\second}$.


==> format.tex <==
% -*- mode: latex -*-
% This contains format control, mostly hackings for more space.

\makeatletter
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{0.2ex \@plus 0.1ex \@minus .3ex}{-0.5em}%
  {\normalfont\normalsize\bfseries}%
} 
\makeatother
% \DefineFNsymbolsTM{myfnsymbols}{% def. from footmisc.sty "bringhurst" symbols
% 	\textasteriskcentered *
% 	\textdagger    \dagger
% 	\textdaggerdbl \ddagger
% 	\textsection   \mathsection
% 	\textbardbl    \|%
% 	\textparagraph \mathparagraph
% }%
% \setfnsymbol{myfnsymbols}
% %%% packages added for appendix.
% %boxruled, ruled, tworuled, plain
% %vlined, lined, noline
% %noend

\newcommand{\realnewpage}{\onecolumn\twocolumn}

%%%
%%%  Fonts
%%%
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% \usepackage{newtxtext,newtxmath}                        % Times/Times-like math symbols
\usepackage{bm}
\usepackage{courier}
\usepackage[scaled=0.92]{helvet}
\usepackage{balance}



%%%
%%%  Space on section headings
%%%
% \usepackage[compact]{titlesec}
% \usepackage{titlesec}
% \titleformat{\paragraph}
%     {\normalfont\bfseries}
%     {}
%     {}
%     {}
% \titlespacing{\paragraph}{0pt}{*1}{*1}      % SPACE
% \titlespacing{\section}{0pt}{2pt}{2pt}      % SPACE
% \titlespacing{\subsection}{0pt}{1pt}{1pt}      % SPACE
\titlespacing\section{0pt}{10pt plus 4pt minus 2pt}{5pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{10pt plus 4pt minus 2pt}{5pt plus 2pt minus 2pt}
\titlespacing\subsubsection{0pt}{10pt plus 4pt minus 2pt}{5pt plus 2pt minus 2pt}
%\titleformat{\section}%                     % IEEE/ACM: caps + period
%  {\bf\large\uppercase}{\thesection.\quad}{0pt}{}



%%%
%%%  Space between figure and caption (assuming caption
%%%  is below figure)
%%%
%\usepackage[font=bf,aboveskip=0pt]{caption} % SPACE
%%  Space between caption and body text of document
%\addtolength{\textfloatsep}{-7pt} % SPACE

%%%
%%%  Space control for Lists
%%%
\usepackage{enumitem}
\setlist{itemsep=0pt,parsep=0pt}             % more compact lists

%%%
%%%  Space control for Header / Footer
%%%
\usepackage{fancyhdr}
\renewcommand{\headrulewidth}{0pt}

%%%
%%%  Some other space savor.
%%%

%\usepackage{titling}
%\setlength{\droptitle}{-5em}   % This is your set screw
%\setlength\floatsep{10pt}
%\setlength\textfloatsep{10pt}
%\setlength\intextsep{10pt}
%\setlength{\abovecaptionskip}{2pt}
%\setlength{\belowcaptionskip}{0pt}

%%%
%%%  Misc
%%%
%\usepackage[pdftex]{graphicx}
%\usepackage{soul}
% this allows \st and friends to work with citations
%\soulregister\cite7
%\soulregister\ref7
%\soulregister\pageref7

%\setlength{\parindent}{0pt}
%\setlength{\parskip}{\baselineskip}

%\clubpenalty=10000  % Don't allow orphans
%\widowpenalty=10000 % Don't allow widows


%%%
%%%  Footnotes / Endnotes
%%%
\interfootnotelinepenalty=10000  % Split footnotes are annoying


%%%
%%% fixing bug of section number missing on some Ubuntu distro.
%%%
% \usepackage{etoolbox}
% \makeatletter
% \patchcmd{\ttlh@hang}{\parindent\z@}{\parindent\z@\leavevmode}{}{}
% \patchcmd{\ttlh@hang}{\noindent}{}{}{}
% \makeatother
% %%% end fixing
% 
% 
% \ifthenelse{\equal{\PAGENUMBERS}{yes}}{%
%   \pagestyle{plain}
% }{%
%   \pagestyle{empty}
% }

%%%
%%%  Page Setup
%%%  OSDI 16: 6.5 * 9, with 0.25 column sep.
%%%  SOSP 17: 7 * 9, with 0.33 column sep.
%%%
%\special{papersize=8.5in,11in}
%\setlength{\pdfpagewidth}{8.5in}
%\setlength{\pdfpageheight}{11in}

\usepackage{ifthen}
%\ifthenelse{\equal{\PAGENUMBERS}{yes}}{%
%  \usepackage[nohead,
%            left=0.75in,right=0.75in,top=1.0in,
%            footskip=0.5in,bottom=1in,     % Room for page numbers
%            columnsep=0.33in
%            ]{geometry}
%}{%
%\usepackage[noheadfoot,left=0.75in,right=0.75in,top=1.0in,
%            footskip=0.5in,bottom=1in,
%            columnsep=0.33in
%	    ]{geometry}
%}


%%%
%%% Uncomment next line if your printer outputs black
%%% boxes instead of drop shadows; older PDF interpreters
%%% in printers can't handle those PDF 1.5 features
%%%
%\pdfminorversion=3
%\pdfobjcompresslevel=2




%%% Color box for the Raft summary
\usepackage{tcolorbox}
%\usepackage[dvipsnames]{xcolor}

\usepackage{titling}
\setlength{\droptitle}{-4em} % remove the extra space above title

==> futurework.tex <==
% \vspace{-0.48cm}
% \section{Future Work}
% \label{discussion}

% % SmartNICs for timestamp like in Octopus
% % Private DCs built for stock exchanges like the CME-GCP collaboration
% % Microsoft’s hollow fiber acquisition.
% % Maybe using FPGA instances.
% % Design with the support of cloud provider
% % Use of RDMA?

% In on-premises exchanges, some MPs implement their trading algorithms on FPGA to achieve low-latency processing. An interesting question is whether FPGA instances in the cloud~\cite{fpga_aws} can serve the same purpose. In AWS, FPGAs do not have direct network access; instead, an associated VM receives the packets and then forwards them to the FPGA. This raises uncertainty about whether FPGA-based low-latency processing of orders is feasible in such an environment. Similarly, whether the \sysname{} proxies can be offloaded to FPGAs is an interesting direction for enhancing performance. 

% Finally, in \sysname{}, we have assumed that cloud providers do not offer any additional support to tenants for building financial exchanges. However, if a cloud provider were to grant access to the underlying infrastructure, it could lead to better performance, such as improved clock synchronization and the use of SmartNICs for fairness~\cite{octopus_google}.

==> goals.tex <==
\vspace{-0.32cm}

%Our main goals are to: (i) develop a scalable multicast service, (ii) develop an order submission service that handles bursty orders, and (iii) ensure security guarantees comparable to on-premises exchanges. The multicast service must deliver low-latency, and fairness in data delivery to ensure fair trading. The order submission service should manage order bursts effectively to reduce packet drops and maintain high ME throughput. Lastly, strong security boundaries are essential to foster trust in \sysname{} and encourage stakeholder participation. In the following we present an overview of \sysname{} that achieves the above goals. 

% \subsection{Primary Goals}

% % \Para{Goal 1: Scaling Multicast Service for Market Data.}  We target achieving a scale of up to 1000 multicast receivers to meet the demands of modern financial exchange systems~\cite{??}. At such a large scale, latency spikes occur more frequently and becomes the headache to our service. Therefore, \sysname needs to address the latency spikes to build a scalable, fair, and low latency multicast of market data.

% \Para{Goal 1: Scalable Multicast} We aim to build a low latency and fair multicast service that scales to 1,000 receivers. 

% % \Para{Goal 2: Handling Burstiness of Order Submission.} Our second goal is to handle bursts of orders so that the matching engine operates at optimal throughput and the latency of orders is kept to a minimum. 
% \Para{Goal 2: Handling Burstiness of Order Submission.} Efficiently handling sharp and unpredictable bursts of orders from a large number ($\approx1,000$) of MPs is paramount to an exchange. 

% \Para{Goal 3: Enforcing Security Guarantees.} We need to provide the same security abstraction as on-premises exchanges --  MP's proprietary algorithms are secured and correctness of an exchange's operations do not rely on MPs' actions.  


==> inbound_unfairness.tex <==
- the definition of unfairness used by CloudEx is coarse grained
- using LOQ requires a fine grained definition
- LOQ intentionally delays noncritical stuff even if it was generated earlier than some critical stuff
- what really matters is that for a particular price, orders generated early should be prioritized
- so the fine grained definition: old defintion applied per price level


without bursts
- 100 receivers, delay parameter (mine) = 1000, unfariness les than 5\%

with burst:
need to implement DDP

perhaps we should leave this as an open question as I dont think even the new definition is sufficient


imagine
- a proxy that has an order with price p1 and generation time t1 and has no other orders
- and another proxy which has a lot of orders with price p2, time t2 and one order with price p1 and time t0
- where p2 is closer to mid price and t0 < t1 < t2

the ME sequencer is going to receive order <p1, t1> from the first proxy and then only a lot of time later will receiver order <p1, t0> from the second proxy because the second proxy was busy relaying critical orders <p2, t2>

this will lead to unfairness for price level p1 with our new definition as the delay parameter can never account for this: the lateness is due to the presence of critical orders on the second proxy



and the delay parameter should not be end to end because god knows how much time is spent in the LOQ

it should be just receive time and it is good enough




==> interfaces.tex <==


\subsection{Usability}
\label{sec:api}

For the sake of high performance, \systemname{} implements the message processing logic by fully using DPDK. However, we also realize that many legacy applications are programmed based on the POSIX socket APIs, and porting them to the DPDK-based APIs is costly and challenging. So we implement a second interface with UNIX sockets at the sender and receivers.\footnote{Proxies between sender and receivers are still implemented with DPDK.} To minimize the performance sacrifice, we leverage eBPF to reduce several overheads.

First, the sender, instead of sending $F$ messages to Layer-0 proxies, sends one message using a UNIX socket which is then captured by an eBPF/TC hook. The hook replicates the message using $bpf\_clone\_redirect()$ and sends one copy to each of the $F$ Layer-0 proxies. This eliminates the overhead of creating message copies in the userspace and sending each copy to the kernel. 

Second, receivers install an eBPF/XDP hook which makes sure that the earliest copy of a multicast message is received and sent to the application. The later copies are dropped by the hook. Due to hedging, a receiver gets $H+1$ copies of a multicast message where the earliest one is supposed to be accepted. The XDP hook serves that purpose. This optimization keeps duplicate messages from traversing the kernel stack and going to userspace. However, implementing a packet de-duplication mechanism is challenging in XDP as only fixed-length buffers are allowed and several operations (e.g., modulo (\%)) are not permitted. So we devise an algorithm that works under the assumption that messages that are sent by the sender one second apart do not get re-ordered. Details of our de-duplication implementation are described next. 

We start with a fixed-length buffer $B$ of size N where N equals the smallest power of 2 that is greater than or equal to the message rate, $R$ (i.e., $R$ messages per second). This restriction on $N$ allows us to implement a modulo operation, not allowed in XDP, as a bitwise operation which is allowed in XDP. The buffer is implemented as a bpf\_map of size $N$. Algorithm \ref{alg:pkt_dedup_xdp} shows how we achieve packet de-duplication and only accept the packet copy that is received earliest and discard the rest. 


\begin{algorithm}
\caption{Packet De-Duplication with a Fixed-Length Buffer}
\label{alg:pkt_dedup_xdp}
\begin{algorithmic}[1]
    \State \textbf{Input:} Message ID ($id$), Buffer $B$ of size $N$
\Procedure{PacketDeduplication}{$id, B, N$}
    \State $index \gets id \And (N-1)$
    \If{$B[index] < id$}
        \State $B[index] \gets id$
        \State \textbf{Accept} the message
    \ElsIf{$B[index] == id$}
        \State \textbf{Discard} the message as a duplicate
    \Else
        \State \textbf{Error:} $B[index] > id$ \Comment{Assumption Violated}
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}
% Our algorithm is accurate under this assumption.

% A multicast sender has to send messages to the top-level $F$ proxies of a \systemname{} tree, and each multicast receiver receives copies of messages from $H+1$ proxies where a receiver only accepts the earliest copy. The most performant way to interact with the service is that the multicast sender and receivers use DPDK. However, there can be scenarios where the use of kernel bypass is not a suitable option so we provide another high-performance interface: Unix Sockets + eBPF. This interface trades off some performance for usability, allowing developers to easily engage with \systemname{} and evaluate it before committing to use it.

% \textbf{Sockets + eBPF interface:} The multicast sender installs an eBPF/TC hook in the kernel and then uses unix sockets. This way the sender has to send the message to only one proxy. The message is captured by the eBPF/TC hook where it is replicated using bpf\_clone\_redirect() with very low overhead and sent to all the first-level proxies of the \systemname{} tree. Similarly, a multicast receiver installs an eBPF/XDP hook in the kernel and uses unix sockets for receiving messages. The eBPF/XDP hook ensures that only the earliest copy of a multicast message is received by the receiver and the rest are discarded. This message de-duplication by the eBPF/XDP hook poses an interesting problem. How to check that a received message has an ID that has been previously seen? Although each message has an associated message ID, an XDP program cannot allocate memory to implement a set or hashmap functionality and may only use fixed-length eBPF maps. An alternative solution is to use bloom filters and tolerate false positives. Our mechanism provides perfect accuracy but requires an assumption about packet re-ordering we explain next. 

% \textbf{De-duplication with a fixed-length buffer:} We provide a mechanism to implement a set membership check using a fixed-length buffer in eBPF/XDP. The main assumption that enables this is that packet re-ordering should not interleave packets that are sent a second apart. A similar assumption has been made in \cite{sprout} albeit in a different context where packets sent 10 milliseconds apart are assumed to never get re-ordered. 

% We start with a fixed-length buffer $B$ of size N where N equals the smallest power of 2 that is greater than or equal to the message rate, R (i.e., R messages per second). This restriction on N allows us to implement modulo operation, not allowed in XDP, as a bitwise operation. The buffer is implemented as a bpf\_map of size N. Algorithm \ref{alg:pkt_dedup_xdp} shows how we achieve packet de-duplication and only accept the packet copy that is received earliest and discard the rest. 

==> limitations.tex <==
\vspace{-0.3cm}
\section{Limitations \& Future Work}
\label{limitations}
\label{discussion}

If all MPs receive a message within \SI{1}{\micro\second} of each other, we consider it fairly disseminated. However, in on-premises exchanges, fairness guarantees are more precise, down to the level of nanoseconds. Achieving such fairness requires synchronizing the clocks of all receiver VMs with accuracy better than nanoseconds—a level of precision that current public cloud technology does not yet provide.

\sysname{} uses UDP for both multicast and order submission. The reliability required for order submission has not been fully explored. With pacing in place, we envision utilizing OnRamp like congestion control that handles transient bursts. 

In on-premises exchanges, some MPs implement their trading algorithms on FPGA to achieve low-latency processing. An interesting question is whether FPGA instances in the cloud~\cite{fpga_aws} can serve the same purpose. In AWS, FPGAs do not have direct network access; instead, an associated VM receives the packets and then forwards them to the FPGA. This raises uncertainty about whether FPGA-based low-latency processing of orders is feasible in such an environment. Similarly, whether the \sysname{} proxies can be offloaded to FPGAs is an interesting direction for enhancing performance. 


==> notes.tex <==
1) Write a section about the security problem
1a) Explain different models like i) separate gateway, ii) trader owns receiver, iii) exchange owns receiver or iv) just trader trusting the exchange
1b) Explain how it comes at the cost of latency and an enlarged delivery window
1c) It would require two levels of hold and release, a destination-based and a source-based


2) Write about where the variance comes from: transmission and network. Transmission one is small and can be eliminated by fanout/message sizes, network one needs to be eliminated by hold-release. Playing with Message sizes has its own problems

3) 

==> old_intro.tex <==
% \vspace{-0.1cm}
% \section{Introduction}
% Financial exchanges are interested in migrating to the public cloud to improve scalability, increase geographic presence, bring in more participants, reduce costs, and alleviate management strain~\cite{nasdaq_aws_partnership,google-invest-financial-exchange, dbo_prateesh, octopus_google, cloud_democratize, cloudex-hotos}. Currently, such exchanges operate in private data centers or colocation facilities~\cite{colocation} that are heavily engineered for deterministic (i.e., low variance) performance. By contrast, public cloud tenants have limited control over the network fabric, an impediment to realizing the requirements of an exchange on the public cloud. In general, two major networking challenges confront a cloud-native exchange.

% The first challenge is to build a \emph{fair} and \emph{low-latency} multicast service for market data. Market data contains information about different market activities which is used by market participants (MPs) for making trades. MPs often compete on how quickly they can react to some piece of market data. The multicast service needs to have as low latency as possible so that MPs trade on the most up-to-date information, and the service needs to be \emph{fair} in data delivery to enable fair competition among the MPs. Here fairness\footnote{This latency-centric concept of fairness is distinct from standard networking notions of fairness like Jain’s index, etc., which are throughput-centric.} requires simultaneous delivery of data to the MPs so that no MP has an advantage over the others while making trades. Realizing these requirements in the public cloud is challenging as the cloud is an inherently non-deterministic medium where the performance of VMs and latency between VMs can vary because of factors not in the control of a cloud tenant e.g., noisy neighbor problems, VM migrations, etc. 

% The second challenge is efficiently processing trading orders submitted by MPs in response to market data. Sharp bursts of order submissions~\cite{sharp_bursts} can cause packet losses and increased trade latency. The matching engine (ME) on the exchange server receives and matches bids (buy offers) with asks (sell offers). High ME throughput and low latency are crucial for efficient financial exchanges. However, provisioning sufficient resources for worst-case scenarios like order bursts negates the cost and elasticity benefits of cloud.

% %Quick overview of architecture
% We design and implement \sysname{}, a scalable cloud-hosted financial exchange. \sysname{} has two main components: a fair multicast service (on the exchange outbound side) and, an order submission service (on the exchange inbound side). 
% We use an overlay tree of proxies as a starting point in our design where the exchange server is at the root of the tree and the MPs are the leaves. A tree helps in scaling message delivery to a large number of receivers while bounding the latency. We incorporate our techniques in the tree to build a multicast and an order submission service. 

% On the exchange outbound side, we implement cloud-focused overlay techniques, aimed at reducing multicast latency, minimizing latency differences across receivers, and ensuring predictable performance despite latency fluctuations inherent to the public cloud. These goals set \sysname{} multicast apart from traditional approaches in the multicast literature. To achieve deterministic low latency in the cloud, our main insight is to hedge the risk of each system component experiencing performance variance. This motivates the design of the following three techniques. To minimize the effects of latency spikes on the links between VMs, we introduce \textit{round-robin packet spraying} in the overlay tree where each parent proxy changes the set of its children after every message. This reconfiguration prevents any single path from being used consecutively, reducing the impact of transient latency spikes. For countering latency fluctuations introduced because of proxy VMs (or the hosts), we introduce \textit{proxy hedging}. Each node in the tree has two parent proxies and a child node (a proxy or an MP VM) only processes a message that is received earlier and discards the second. Lastly, we introduce \textit{receiver hedging} where each MP is assigned two receiver VMs that run the same state machine (of a trader’s trading algorithm). With high probability, at least one receiver VM for each trader will receive multicast messages with minimal latency and no fluctuations.

% On the exchange inbound side, we use the same proxy tree in reverse to manage incoming orders from MPs. Orders are relayed from the leaves/MPs to the root/ME through proxies, reducing incast congestion at the ME by lowering the fan-in factor compared to not utilizing a tree.
% Moreover, during burst periods, proxies dynamically pace packets to prevent drops~\cite{onramp} as it moves the packet queues from the network to the proxies. This allows for a smart scheduling policy to enhance the order matching rate of ME. We design a distributed packet scheduling policy that runs on each proxy in the tree, prioritizing "critical" packets as they are relayed to ME. We implement this with a priority queue called the Limit Order Queue (LOQ), which identifies packets containing critical trading orders based on their likelihood of being matched upon arrival at ME. Since some orders cannot not be immediately matched depending on other available orders (\S\ref{subsec:ex_op_overview}), those orders can afford to arrive at the exchange slightly later. The LOQ significantly enhances an exchange's performance during bursts by reducing order latency and enhancing its order matching rate.

% Furthermore, we need to realize the same trust model that on-premises exchanges provide to the traders. In such a trust model, the exchange and traders have a clear separation of security boundaries and the traders' actions do not impact an exchange's operations. We present three trust models and show their performance vs security trade-offs. 

% \Para{Evaluation.} We show that latency difference between 1,000 multicast receivers can be minimized to $\leq\SI{1}{\micro\second}$, which achieves simultaneous delivery of market data while bounding median multicast latency to \SI{250}{\micro\second}. \sysname{} scales better and achieves 50\% lower latency compared to a multicast service provided by AWS (called AWS TGW-based multicast). We efficiently handle large bursts of orders, nearly doubling a matching engine’s order matching rate (compared to not utilizing LOQ). Finally, while \sysname{} significantly outperforms the baseline solutions, its performance falls short of that achieved by on-premises financial exchanges (\S\ref{limitations}). Nevertheless, we push the boundaries of the performance guarantees that financial exchanges can reliably achieve on the public cloud, which is already sufficient for various types of trading activities. 

==> oldorders_submission.tex <==
\section{Inbound Communication}
\label{exchange_inbound}
% \vspace{-0.24cm}

The matching engine (ME) is located at the root VM of the tree, while orders come from leaf nodes (MPs/traders). Using the proxy tree in reverse for order submission helps reduce the submission load on the ME. Intermediate proxies gather orders from multiple downstream nodes and forward them upstream, so the root VM simultaneously processes packets from only $F$ proxies instead of $N$ MPs. The reduced fan-in decreases packet losses. In a benchmark with 10 VMs each submitting 5K orders per second to the ME, the packet loss rate is 1.58\%. Adding two intermediate proxies to create a tree structure lowers this loss rate to 0.68\%, as the proxies alleviate incast congestion by relaying orders to the ME.

% %% This para seems to be redundant
% To tackle order bursts, we need to first handle packet losses, which can easily happen because of the bursty many-to-one communication when orders traverse up the tree to reach ME. Using a tree helps mitigate the incast congestion but it does not completely eliminate the problem. We employ packet pacing at the intermediate proxies to shape the outgoing traffic from the proxies to minimize the packet drops. 

A tree alleviates some incast congestion, but is not sufficient especially when order bursts occur. We use packet pacing at the proxies to tackle such bursts. Avoiding drops by pacing the packets comes at the cost of filling up queues at the proxies which may increase order submission latency. To maintain low latency for orders and achieve high order matching rate of ME, we design a distributed packet scheduling policy, implemented at the proxies. The policy, realized through a priority queue, Limit Order Queue (LOQ), prioritizes orders that have prices closest to the current mid-price. 

% \vspace{-0.3cm}
\subsection{Pacing Outgoing Packets}
% \vspace{-0.24cm}
Proxies continuously request the OWD estimates of packets sent to parent proxies or the ME. An increasing OWD is an indicator of congestion at the receiver (i.e., parent proxy or ME) and the proxies use this to slow down -- increase the interpacket duration -- to avoid packet drops.

Aggressive pacing can lead to bandwidth underutilization, while insufficient pacing risks excessive packet drops due to congestion. Ideal pacing balances these concerns by optimizing bandwidth usage, and adjusting pacing to avoid drops during bursts while reclaiming bandwidth once bursts vanish. In \sysname{}, prioritizing drop prevention is more important than operating at the maximum bandwidth. Sharding techniques for MEs can improve throughput~\cite{cloudex-hotos}, hence our focus is on minimizing packet drops during bursts. Nonetheless, it is favorable to utilize as much of the throughput as possible if it does not introduce substantial packet loss.

Our pacing heuristic calculates an amount of time to wait before sending the next packet (the pacing quantum) based on how much the most recent OWD estimate ($e$) deviates from a threshold OWD $T$. $e$ is computed as the median OWD of all the packets sent in the last \SI{50}{\milli\second}.
% \[
% P_{\text{new}} =
% \begin{cases} 
% P_{\text{old}} + 20 & \text{if } e \geq T + 10 \\
% P_{\text{old}} - 10 & \text{if } e + 10 \leq T \\
% P_{\text{old}}      & \textit{otherwise}
% \end{cases}
% \]
The heuristic increases the pacing quantum by \SI{20}{\micro\second} if $e$ increases by \SI{10}{\micro\second} over $T$. And the quantum is decreased by \SI{10}{\micro\second} if $e$ falls below $T$ by \SI{10}{\micro\second}. The heuristic is aggressive in increasing the pacing as compared to when decreasing the pacing because it is critical to avoid packet drops. When $e$ is sensed to be decreasing below $T$, we \textit{slowly} (decrease by \SI{10}{\micro\second} vs increase by \SI{20}{\micro\second}) decrease the pacing to reclaim the available bandwidth. A sudden decrease is avoided to account for imperfect estimates. After pacing is applied, we empirically observe that we maintain a stable throughput (orders received per second) at the ME, despite being confronted by bursts of orders. We also observe that pacing significantly reduces packet drops.  In \S\ref{evals_pacing}, we show pacing can achieve a reasonable balance between throughput and packet losses. Our attempts to further improve this simple pacing heuristic were not fruitful because of the noise inherent in calculating $e$ as a cloud tenant. It is possible that there are better pacing schemes that Pareto dominate our scheme on throughput and loss; for now, though, we have found our simple scheme to suffice.

\Para{Parameter Selection} We pick $T$ and the increase and decrease amounts offline by running a control experiment where VMs communicate at a fixed rate which is expected to be the equilibrium rate for order submission. 

% \vspace{-0.5cm}
\subsection{Limit Order Queue (LOQ)}
% \vspace{-0.24cm}
LOQ implements a distributed scheduling policy across all proxies of the overlay tree, improving ME's order matching rate and reducing order latency. Its benefits are pronounced when packet queues form at the proxies. 

LOQ leverages the observation that orders with prices far from the mid-price tend to wait in the LOB, even if they arrive earlier than orders closer to the mid-price. These noncritical orders can afford to remain in proxy queues without impacting the matching process. If a proxy knows the mid-price, it can prioritize outgoing orders based on their proximity to this price. Critical orders—those closer to the mid-price and more likely to be matched—are relayed to the ME first. This prioritization boosts ME throughput (orders matched per second) and reduces the latency of matched orders.

The above approach to LOQ relies on proxies having access to mid-price information. One way to provide this information is for the ME to periodically multicast the mid-price to all proxies, which would increase the ME's workload, especially during times of high activity and order overloads. Another solution is for each proxy to maintain an approximate LOB based on the orders it \textit{relays} to the ME. However, this adds the overhead of maintaining an LOB at the proxies and may diminish the benefits of LOQ if a proxy's LOB significantly diverges from the ME's LOB.

\Para{Mid-price agnostic LOQ:} To avoid maintaining mid-price information at each proxy, we design LOQ to be agnostic of the mid-price information. A proxy needs to prioritize some orders over others based on their probability of getting matched as they arrive at ME. The distance to the mid-price is a good indicator of this probability. However, a proxy does not need the exact probability but just the ordering relationship i.e., whether the probability of one order is higher or lower than some other order that it has in the queue. We leverage this to design a mid-price agnostic LOQ as follows. 

LOQ at each proxy consists of two separate priority queues, one for bids and one for asks. The bids queue sorts the orders by price in descending order while the asks queue sorts the orders by price in ascending order. This reflects the ME behavior that the highest bid and lowest ask are selected for a potential match. A proxy consults the two priority queues in a round-robin fashion for dequeuing the orders and forwarding them to ME. This design eliminates the need for mid-price information at the proxies, simplifying the system. 

LOQ also needs to respect price-time-priority that an ME uses for order matching. Each priority queue at the proxies first sorts the orders by price, as discussed above, and then by order generation timestamp, $t_g$. This ensures that when a proxy dequeues an order from LOQ for relaying to ME, another order with the same price and lower $t_g$ does not exist in the queue. A sequencer delay $d_s$ is used by ME to account for any network reordering: An ME only dequeues an order for processing if it was received at least $d_s$ \SI{}{\micro\second} ago which gives enough time, with high probability, to the other orders to arrive and get prioritized if they deserve to do so e.g., they have a lower $t_g$ or an LOQ deemed it to arrive at ME earlier.
%CloudEx proposed an online technique to tune $d_s$ to reach desired level of unfairness, we do not expand on it as it can be naively imported to \sysname{}.

% In summary, an LOQ has a three step dequeue mechanism: (i) consult bids and asks queues in a round-robin fashion, (ii) in each queue, prioritize by price and then (iii) by order generation timestamp. 

\subsection{Deconstructing LOQ}
% \vspace{-0.24cm}
LOQ improves order matching rate and reduces latency of matched orders by reordering queues at the proxies. A natural question is whether we are sacrificing \textit{correctness} by such reordering. The reordering only aims to prioritize orders with a higher likelihood of getting matched, i.e., those with a lower chance of remaining in the LOB and idling the ME upon arrival at the ME. Intuitively, it seems LOQ does not affect the matching behavior of ME, but we have not formally shown that. Empirically, we use \textit{inbound fairness}\footnote{Inbound fairness is distinct from the (outbound) multicast fairness} to quantify how much LOQ changes the behavior of ME.

\Para{Inbound fairness}: For an ME, it's critical to ensure that orders generated earlier are matched before those generated later if both provide the same market value. This concept of \textit{inbound} fairness is a key feature of matching algorithms like price-time priority. Any infrastructure for exchanges needs to ensure an ME can do the above: \textit{if an order submitted earlier ($o_1$) should be matched before a later order ($o_2$) then the ME should have received both by the time it chooses $o_2$ for execution}. 

CloudEx~\cite{cloudex-hotos} proposed \textit{inbound unfairness ratio} to quantify the inbound fairness. The ratio is calculated as the percentage of sequenced\footnote{a sequencer sequences all the orders based on their generation timestamp} orders received out-of-order by the ME. We find that LOQ shows very poor inbound unfairness ratio ($>= 70\%$, where ideal value is 0\%). Upon interrogation, we realize the CloudEx's definition is unnecessarily strict. It may increase unfairness ratio under a benign scenario: an order $o_1'$ with order generation timestamp, $t_g=t_1'$ arrives later than $o_2'$ with $t_g=t_2'$ where $t_1' < t_2'$ but $o_2'$ has a price much closer to the mid-price while $o_1'$ has a price farther away and would only wait in the LOB even if it arrives at ME earlier than $o_2'$. This is the exact scenario which LOQ takes advantage of. 

We realize the issue with CloudEx's definition, and propose a new one: \textit{order matching fairness}. Assume MPs attach $t_g$ with each order they submit.\footnote{Security issues with timestamping are addressed in \S\ref{sec:trust_model}.} In \textit{order matching fairness}, an order with $t_g = t$ and price $p$ is only considered unfairly treated if it arrives at the ME and an order with $t_g = t'$ and price $p'$ has already been matched by ME where $t' < t$ and $p = p'$. The percentage of unfairly treated orders among the total matched orders constitute inbound unfairness ratio. 

By focusing on the \textit{matching} of orders and \textit{price}, the order matching fairness allows packet scheduling policies to send orders, to ME, with different prices out of sequence to enhance metrics like the order matching rate. We believe our new inbound fairness definition captures the true intent of inbound fairness, however we lack a formal analysis, which is left for future work. In \S\ref{fancypq_evals}, we find that \sysname{} leads to small inbound unfairness ratio which remains unchanged with or without LOQ, suggesting that LOQ may not affect correctness. 

==> preamble.tex <==

% % to be able to draw some self-contained figs
% \usepackage{amssymb}
% % inlined bib file
% \usepackage{filecontents}
% \usepackage{adjustbox}
% \usepackage{babel}
% \usepackage{ifoddpage}
% \usepackage{pifont}
% \usepackage{siunitx}
% \usepackage{multirow}
% \usepackage{adjustbox}
% % to be able to draw some self-contained figs
% \usepackage{tikz}
% \newcommand*\circleincap[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {#1}}} }
% \newcommand*\circled[1]{\tikz[baseline=(char.base)]{
%             \node[shape=circle,draw,inner sep=0pt] (char) {#1};}}
% \usepackage{amsmath}
% \usepackage{enumitem}
% \usepackage[most]{tcolorbox}
% \usepackage{multicol,lipsum}
% \usepackage[utf8]{inputenc}
% \usepackage{algorithmicx}
% \usepackage{algorithm}
% %  \usepackage{arevmath}     % For math symbols[cause bad looking of formulas in VLDB]
% \usepackage{tabularx,booktabs}
% \usepackage{tabularray}
% \usepackage[noend]{algpseudocode}
% \usepackage{soul}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argminA}{arg\,min} % Jan Hlavacek
% \usepackage{appendix}
% \usepackage{balance}
% \usepackage{makecell}
% \usepackage[skip=4pt]{caption}
% \usepackage{diagbox}
% \usepackage{float}
% \usepackage{graphicx}
% \usepackage{hyperref}
% \usepackage{siunitx}
% \usepackage{subcaption}
% % \usepackage{times}  # It makes title bolder (I don't know why)
% \usepackage{threeparttable}
% \usepackage{url}
% \def\UrlBreaks{\do\/\do-}
% \usepackage{verbatim} 
% \usepackage{xspace}
% \usepackage{xcolor}
% % % % total number of pages
% \usepackage{totpages}
% %\usepackage{authblk}
% \usepackage{mathtools}
% \usepackage{physics}
% \usepackage{array}
% \usepackage{pdfpages}
% \usepackage{adjustbox}
% \usepackage{lipsum}
% \usepackage{multicol}
% \usepackage{float}
% \usepackage{environ}
% \usepackage[normalem]{ulem}
% \usepackage{hyperref}

% \usepackage{titlesec}
            
% \usepackage{tcolorbox}
% \definecolor{mycolor}{rgb}{0.122, 0.435, 0.698}


==> simaltaneous_delivery.tex <==
\subsection{Simultaneous Delivery}
\label{sec:sim_delivery}

A hold-and-release mechanism was introduced by ~\cite{cloudex-hotos} to achieve simultaneous delivery in the public cloud. This mechanism inflates the latency of messages to some receivers to equalize latency to all the receivers. Multicast messages are stamped with a deadline and the receivers process the messages at or after the deadline. This achieves simultaneous delivery (or processing) of market data by the receivers with high probability, assuming good deadlines. A deadline set too far in the future poses the risk of unnecessarily increasing the latency. A too-small deadline runs the risk of not achieving simultaneous delivery. 

Using ``hold-and-release'' mechanisms for a large number of receivers inflates the latency significantly. However, when used in conjunction with a proxy tree and our techniques to keep latency low, the required inflation is decreased and the overall multicast latency is kept low. Implementing this mechanism for a large number of receivers raises several implementation concerns i.e., aggregating OWD estimates to all the receivers to calculate the deadlines. We use our proxy tree in the reverse direction in an all-reduce manner to get the maximum OWD estimate across all the receivers. We explain our implementation in appendix~\ref{app:sim_delivery}. 

The hold-and-release mechanism also requires the receivers (i.e., MPs) to follow a protocol while MPs have the incentive to violate it. We address this in \S\ref{sec:trust_model}. 

==> symbol_table.tex <==

\begin{table*}[!t]
\centering
\small
\caption{Variables in our multicast model}
\label{tab:variable}
\begin{tabular}{|c|c||c|c|}
\hline
\textbf{Symbol} & \textbf{Meaning} & \textbf{Symbol} & \textbf{Meaning}\\
\hline

$B$ & Ingress/egress  & $L$ & End-to-end latency, i.e., latency from \\
  & bandwidth of a VM & & a sender to the last receiver\\
\hline

$D$ & Number of hops (proxy  & $M$ & Multicast message  \\
  & VMs) between a sender & & size (in bits)\\
  & and receiver & &\\
\hline

$F$ & Fanout factor & $N$ & Number of multicast  \\
  &               &   & receivers \\
\hline

$F_i$ & Fanout size of a node in layer & $p$ & Propagation delay \\
      & $i$ of a multicast tree & &\\
\hline

$i$ & Hop/Layer index & $t$ & Transmission delay \\
\hline

$w$ & Wire-to-wire delay & &\\
\hline

\end{tabular}

\end{table*}
